FlexiBit: Fully Flexible Precision Bit-parallel Accelerator Architecture for Arbitrary Mixed Precision AI

Recent research has shown that large language models (LLMs) can utilize low-precision floating point (FP) quantization to deliver high efficiency while maintaining original model accuracy. In particular, recent works have shown the effectiveness of non-power-of-two precisions, such as FP6 and FP5, and diverse sensitivity to low-precision arithmetic of LLM layers, which motivates mixed precision arithmetic including non-power-of-two precisions in LLMs. Although low-precision algorithmically leads to low computational overheads, such benefits cannot be fully exploited due to hardware constraints that support a limited set of power-of-two precisions (e.g., FP8, 16, 32, and 64 in NVIDIA H100 Tensor Core). In addition, the hardware compute units are designed to support standard formats (e.g., E4M3 and E5M2 for FP8). Such practices require re-designing the hardware whenever new precision and format emerge, which leads to high hardware replacement costs to exploit the benefits of new precisions and formats. Therefore, in this paper, we propose a new accelerator architecture, FlexiBit, which efficiently supports FP and INT arithmetic in arbitrary precisions and formats. Unlike previous bit-serial designs, which also provide flexibility but at the cost of performance due to its bit-wise temporal processing nature, FlexiBit's architecture enables bit-parallel processing of any precision and format without compute unit underutilization. FlexiBit's new capability to exploit non-power of two precision and format led to 1.66x and 1.62x higher performance per area on GPT-3 in FP6 targeting a cloud-scale accelerator, compared to a Tensor Core-like architecture and a state-of-the-art bit-parallel flexible precision accelerator, BitFusion, respectively. Also, the bit-parallel nature of FlexiBit's architecture led to 3.9x higher performance/area compared to a state-of-the-art bit-serial architecture.

==> backup/scratchpad.tex <==
\begin{equation}
Act\_BitMask[i] = (2^{P_M(A) - 1} <<< 1) \times 2^{i \bmod {P_M(A)}}
\end{equation}

\begin{equation}
Act\_OpMask[i] = (2^{\frac{B_M}{P_M(A)} \times P_M(A) \times &P_W(A)} - 1) \times 2^{i \bmod {P_M(A)}}
\end{equation}
%\begin{equation}
%Act\_OpMask[i] = repeat \left[ \left\{ (P_M(A) \times P_M(W) \times \left[\frac{B_M}{P_M(A)} - 1\right]) \{1\text{b}0\}, \ (P_M(A) \times P_M(W)) \{1\text{b}1\} \right\} \right]  << (P_M(A) \times P_M(W) \times \left[\frac{i}{P_M(A)} - 1\right])
%\end{equation}





\begin{equation}
Weight\_BitMask[i] = (2^{P_M(A) \times P_M(W)} - 1 <<< 1) \times 2^{\frac {i}{P_M(A)}}
\end{equation}

%\begin{equation}
%Weight\_BitMask[i] = \text{repeat} \left( \left( P_M(A) \times (P_M(W) - 1) \right)\{1\text{'b}0\}, \ P_M(A)\{1\text{'b}1\} \right) << i \times (P_M(A))
%\end{equation}

\begin{equation}
Weight\_OpMask[i] = (2^{P_M(A) \times P_M(W)} - 1 <<< 1) \times 2^{\frac {i}{P_M(A)}}
\end{equation}

%\begin{equation}
%Weight\_OpMask[i] = (P_M(A) \times P_M(W) \times \left[\frac{B_M}{P_M(A)} - 1\right]) \{1'b1\} << (P_M(A) \times P_M(W) \times \left[\frac{B_M}{P_M(A)} \times i \right])
%\end{equation}
\TODO{check formula. Change representation if not clear}

==> tables/PE_Spec.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Four design choices for FlexiBit Processing Element. Units for all numbers except Tree levels are bits.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \textbf{Design Variants} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E}\\
\hline
Input Register  & 16  & 20  & 24  & 28 & 32 \\
\hline
Mantissa/Exponent register  & 8  & 10  & 12 & 14 & 16 \\
\hline
Primitive Buffer Length  & 64  & 100  & 144 & 196 & 256 \\
\hline
Exp. Adder Length  & 64  & 100  & 144  & 196 & 256 \\
\hline
Accumulator Length  & 32  & 50  & 72 & 98 & 128 \\
\hline
Position Designator Length  & 32  & 50  & 72  & 98 & 128 \\
\hline
Max. FBRT Level  & 6  & 6  & 7  & 7 & 8 \\
\hline
Shift Tree Level  & 5  & 5  & 6 & 6 & 7 \\
\hline

\hline
\end{tabular}
\label{tab:design_variants}
\end{table}

==> tables/tab_arithmetic_intensity.tex <==
%\vspace{-4mm}
\begin{table*}[t]
\caption{The model size and the number of computations (multiply-and-accumulate; MAC) of Transformer-based language models and convolutional neural network-based computer vision models. Language model data are based on the batch size of 1 and the sequence length of 128.}
%\vspace{-1mm}
\label{tab:arithmetic_intensity}
\resizebox{1.0\textwidth}{!}{
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|} 
\hline
\textbf{Models} & \textbf{Model Type} & \textbf{Model Size (FP16)} & \textbf{\# Computations (MACs)} & \textbf{Compute to model size ratio} \\
\hline
ResNet50~\cite{he2016deep}
& Computer Vision
& 51.1 MB
& 8.21 B
& 160.7
\\
\hline
BERT-Base~\cite{kenton2019bert} 
& Language Model 
& 219.0 MB
& 11.2 B
& 51.1
\\
\hline
Llama2-7B~\cite{touvron2023llama}
& Large Language Model 
& 13.4 GB
& 850.0 B
& 63.4
\\
\hline
\end{tabular}
}
\end{table*}

==> tables/tab_datatype_parameters.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Data type parameters}
\vspace{-3mm}
\begin{tabular}{| l | l | }
\hline
\textbf{Parameter} & \multicolumn{1}{c|}{\textbf{Description}} \\
\hline
$BW_M(A)$ & Activation mantissa bit width \\
\hline
$BW_M(W)$ & Weight mantissa bit width \\
\hline
$BW_E(A)$ & Activation exponent bit width \\
\hline
$BW_E(W))$ & Weight exponent bit width \\
\hline
$P(A)$ & Data precision of activation values\\
\hline
$P(W)$ & Data precision of weight values\\
\hline
\end{tabular}
\label{tab:datatype_parameters}
\vspace{-3mm}
\end{table}


==> tables/tab_design_space.tex <==
\begin{table}[t]
\caption{A summary of the model parameters and corresponding design space size of recent language models. NDT refers to the number of decomposable tensors in each layer.}
\label{tab:design_space_size}
\centering
\scriptsize
\begin{tabular}{|l|r|r|r|}
\cline{1-4}
\multicolumn{1}{|c|}{\textbf{Model}} 
& \multicolumn{1}{c|}{\textbf{\# Layers}} 
& \textbf{NDT}
& \textbf{\begin{tabular}[c]{@{}l@{}}Decomposition \\ Design Space\end{tabular}} \\
\hline
Bert-Base
& 12
& 6
& O($2^{18}$) \\
\hline
Bert-Large
& 24
& 6
& O($2^{30}$) \\
\hline
Llama 2 - 7B
& 32 
& 5                                                                    & O($2^{37}$) \\ 
\hline
Llama 2 - 70B  
& 80
& 5
& O($2^{85}$) \\ 
\hline
\end{tabular}
\end{table}
